Technical Report: A Trace-Based Performance Study of Autoscaling Workloads of Workflows in Datacenters

To improve customer experience, datacenter operators offer support for simplifying application and resource management. For example, running workloads of workflows on behalf of customers is desirable, but requires increasingly more sophisticated autoscaling policies, that is, policies that dynamically provision resources for the customer. Although selecting and tuning autoscaling policies is a challenging task for datacenter operators, so far relatively few studies investigate the performance of autoscaling for workloads of workflows. Complementing previous knowledge, in this work we propose the first comprehensive performance study in the field. Using trace-based simulation, we compare state-of-the-art autoscaling policies across multiple application domains, workload arrival patterns (e.g., burstiness), and system utilization levels. We further investigate the interplay between autoscaling and regular allocation policies, and the complexity cost of autoscaling. Our quantitative study focuses not only on traditional performance metrics and on state-of-the-art elasticity metrics, but also on time- and memory-related autoscaling-complexity metrics. Our main results give strong and quantitative evidence about previously unreported operational behavior, for example, that autoscaling policies perform differently across application domains and by how much they differ.

==> 7_at_scale_experiment.tex <==
\section{Autoscalers at Scale Experiment}
\label{sct:at_large_experiment}

As it's infeasible to acquire a large amount of resources to conduct real-world experimentation, simulation offers a setting in which system can be tested at scale.
In this experiment we test the three fastest autoscalers managing 100,000 sites.
With this experiment we strive to gain insight into the research question \emph{How well do autoscalers perform on large scale?}.

Our main result in this section is:
\begin{itemize}
	\item \todomihai{Fill in}
\end{itemize}

\subsection{Setup}
In this experiment we run 100,000 sites each with 70 resources.
We duplicate the T4 workload 975 times to obtain an average system utilisation of around 70\%, for the same reason stated in Section~\ref{ssct:setup_bursty_workload_experiment}.

To limit the runtime of this experiment, we run the three fastest autoscalers: react, adapt and reg.
These three autoscalers were chosen based on their algorithmic complexity \todomihai{Include table with the static big O runtimes and memory statistics}.

The Askalon EE2 trace contains a burst of incoming tasks at the start.
Prior work shows bursts can lead to workflow engines running out of different kind of resources \cite{stratan2008performance}.
By measuring the amount of instructions and memory items... 

\begin{figure}[t]
	\hspace*{-1cm} 
	\includegraphics[width=1.1\columnwidth]{figures/2017-11-31_16-09-10_scale_experiment_fill.png}
	\caption{Simulator memory usage over time.}
	\label{fig:scale_fill_experiment_result}
\end{figure}

\begin{figure}[t]
	\hspace*{-1cm} 
	\includegraphics[width=1.1\columnwidth]{figures/2017-11-31_16-09-10_scale_experiment_no_fill.png}
	\caption{Simulator memory usage over time.}
	\label{fig:scale_no_fill_experiment_result}
\end{figure}

\subsection{Results}
We measure the \todoall{what is a good scalability metric?} which shows...
The results are visible in Figure \todoall{make figure and continue text}
